A Categorical Semantics of Fuzzy Concepts in Conceptual Spaces

We define a symmetric monoidal category modelling fuzzy concepts and fuzzy conceptual reasoning within G\"ardenfors' framework of conceptual (convex) spaces. We propose log-concave functions as models of fuzzy concepts, showing that these are the most general choice satisfying a criterion due to G\"ardenfors and which are well-behaved compositionally. We then generalise these to define the category of log-concave probabilistic channels between convex spaces, which allows one to model fuzzy reasoning with noisy inputs, and provides a novel example of a Markov category.

==> eptcsdata.tex <==
\providecommand{\firstpage}{306}
\providecommand{\publicationstatus}{K. Kishida (Ed.): Fourth International Conference\\
on Applied Category Theory (ACT 2021).\\
EPTCS 372, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.372.22}{10.4204/EPTCS.372.22}}
\pdfoutput=1

